Dielectric microwave resonator with large optical apertures for spin-based quantum devices

Towards a spin-based quantum microwave-optical photon transducer, we demonstrate a low-loss dielectric microwave resonator with an internal quality factor of $2.30\times10^4$ while accommodating optical apertures with a diameter of $8\, \mathrm{mm}$. The two seemingly conflicting requirements, high quality factor and large optical apertures, are satisfied thanks to the large dielectric constant of rutile ($\mathrm{TiO_2}$). The quality factor is limited by radiation loss, and we confirmed by numerical simulation that this dielectric resonator can achieve a quality factor exceeding $10^6$ by extending the height of the resonator enclosure. Using this resonator, we performed both continuous-wave (cw) and pulse electron spin resonance (ESR) spectroscopy on 2,2-diphenyl-1-picrylhydrazyl (DPPH) crystalline powder and P1 centers in a diamond crystal in a dilution refrigerator. The cw ESR spectroscopy demonstrated high-cooperativity and strong spin-resonator coupling with the DPPH and P1 centers respectively, while the pulse ESR spectroscopy successfully measured longitudinal and transverse relaxation times.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
